Gait Recognition in the Wild: A Large-scale Benchmark and NAS-based Baseline

Gait benchmarks empower the research community to train and evaluate high-performance gait recognition systems. Even though growing efforts have been devoted to cross-view recognition, academia is restricted by current existing databases captured in the controlled environment. In this paper, we contribute a new benchmark and strong baseline for Gait REcognition in the Wild (GREW). The GREW dataset is constructed from natural videos, which contain hundreds of cameras and thousands of hours of streams in open systems. With tremendous manual annotations, the GREW consists of 26K identities and 128K sequences with rich attributes for unconstrained gait recognition. Moreover, we add a distractor set of over 233K sequences, making it more suitable for real-world applications. Compared with prevailing predefined cross-view datasets, the GREW has diverse and practical view variations, as well as more naturally challenging factors. To the best of our knowledge, this is the first large-scale dataset for gait recognition in the wild. Equipped with this benchmark, we dissect the unconstrained gait recognition problem, where representative appearance-based and model-based methods are explored. The proposed GREW benchmark proves to be essential for both training and evaluating gait recognizers in unconstrained scenarios. In addition, we propose the Single Path One-Shot neural architecture search with uniform sampling for Gait recognition, named SPOSGait, which is the first NAS-based gait recognition model. In experiments, SPOSGait achieves state-of-the-art performance on the CASIA-B, OU-MVLP, Gait3D, and GREW benchmarks, outperforming existing approaches by a large margin. The code will be released at https://github.com/XiandaGuo/SPOSGait.

==> table_tex/overview_baselines.tex <==
\begin{table}[htbp]
\caption{Overview of adopted baselines, including input data type, number of network layers, dimensions of embedding feature, and loss. $N$ in \#embedding of the GEINet means \#training identities.}
%\vspace{-4mm}
\centering
\begin{center}{\scalebox{0.99}{
\smallskip
\begin{tabular}{c|c|c|c|c}
\hline
%\multirow{2}{*}{Backbone} & \multirow{2}{*}{Loss}  & \multicolumn{3}{|c|}{HDFace} & \multicolumn{3}{|c|}{Cross-Age} & \multicolumn{3}{|c|}{Wild}      \\
%\cline{3-11}
%& & 1e-3 & 1e-4 & 1e-5 & 1e-3 & 1e-4 & 1e-5  & 1e-3 & 1e-4 & 1e-5      \\

Baseline & Input &  \#Layers &  \#Embed.  & Loss  \\

\hline\hline
%GEI & GEI &  &   \\
GEINet & GEI & 4 & $N$ & Softmax  \\
TS-CNN & GEI &  6 & - & 2-cls Cross-entropy\\
GaitSet & Sil. & 10 & 15,872 & Batch All triplet  \\
GaitPart & Sil. & 10 & 4,096 & Batch All triplet   \\
CSTL & Sil. &  &  &    \\
GaitGL & Sil. &  &  &    \\
\hline
PoseGait & 3D Pose & 22 & 512& Softmax\&Center  \\
GaitGraph & 2D Pose & 44 &256 & Contrastive  \\
\hline
\end{tabular}}}
\end{center}
%\vspace{-4mm}
\label{table:config}

%\vspace{-6mm}
\end{table}

%{GEI} baseline averages gait silhouettes over one period/sequence as input. And we use random forest as the classifier.

